Non-planar extensions of subdivisions of planar graphs

Almost $4$-connectivity is a weakening of $4$-connectivity which allows for vertices of degree three. In this paper we prove the following theorem. Let $G$ be an almost $4$-connected triangle-free planar graph, and let $H$ be an almost $4$-connected non-planar graph such that $H$ has a subgraph isomorphic to a subdivision of $G$. Then there exists a graph $G'$ such that $G'$ is isomorphic to a minor of $H$, and either (i) $G'=G+uv$ for some vertices $u,v\in V(G)$ such that no facial cycle of $G$ contains both $u$ and $v$, or (ii) $G'=G+u_1v_1+u_2v_2$ for some distinct vertices $u_1,u_2,v_1,v_2\in V(G)$ such that $u_1,u_2,v_1,v_2$ appear on some facial cycle of $G$ in the order listed. This is a lemma to be used in other papers. In fact, we prove a more general theorem, where we relax the connectivity assumptions, do not assume that $G$ is planar, and consider subdivisions rather than minors. Instead of face boundaries we work with a collection of cycles that cover every edge twice and have pairwise connected intersection. Finally, we prove a version of this result that applies when $G\backslash X$ is planar for some set $X\subseteq V(G)$ of size at most $k$, but $H\backslash Y$ is non-planar for every set $Y\subseteq V(H)$ of size at most $k$.

==> simplextbib.tex <==
\bibitem{BokOpoRicSal} D.~Bokal, B.~Oporowski, R.~B.~Richter and G.~Salazar,
Characterizing 2-crossing-critical graphs, {\tt arXiv:1312.3712}.

\bibitem{DinOpoThoVerlarge} G.~Ding, B.~Oporowski, R.~Thomas and D.~Vertigan,
Large non-planar graphs and an application to crossing-critical graphs,
{\it\JCTB} {\bf 101} (2011), 111--121.

\bibitem{HegTho} R.~Hegde and R.~Thomas,
Non-embeddable extensions of embedded minors,
{\tt arXiv:\allowbreak 1401.2973}.

\bibitem{JohThoGener} T.~Johnson and R.~Thomas,
Generating internally $4$-connected graphs, 
{\it\JCTB} {\bf85} (2002), 21--58.

\bibitem{KawNorThoWolbdtw}
K.~Kawarabayashi, S.~Norine, R.~Thomas and P.~Wollan,
$K_6$ minors in $6$-connected graphs of bounded tree-width,
{\tt arXiv:1203.2171}.

\bibitem{KelVertex}A.~K.~Kelmans,
The concept of a vertex in a matroid, the non-separating cycles and
  a new criterion for graph planarity,
In {\sl Algebraic Methods in Graph Theory}, {\bf 1},
  Colloq.\ Math.\ Soc.\ J\'anos Bolyai (Szeged, Hungary),
  North-Holland {\bf 25} (1978), 345--388.

\bibitem{KelSpecialK4}A.~K.~Kelmans,
Finding special subdivisions of $K_4$ in a graph,
In {\sl Finite and infinite sets},
  Colloq.\ Math.\ Soc.\ J\'anos Bolyai (Eger, Hungary),
  North-Holland {\bf 37} (1981), 487--508.

\bibitem{Kelcfc} A.~K.~Kelmans,
On $3$-connected graphs without essential $3$-cuts or triangles,
{\it Soviet Math.\ Dokl.} {\bf 33} (1986), 698--703.

\bibitem{KelPlanarity} A.~K.~Kelmans,
Graph planarity and related topics,
{\sl Contemporary Math.\ \bf 147} (1993), 635--667.

\bibitem{MahRob} J.~Maharry and N.~Robertson,
The structure of graphs not topologically containing the Wagner graph,
manuscript, 
{\tt https://u.osu.edu/maharry.1/files/2013/05/ \hfil\break
WagnerFreeGraphsSubmittedToJCTBOctober2013-1w1q21n.pdf}.

\bibitem{NorThoLinear}S.~Norin and R.~Thomas,
Linear decompositions of $t$-connected graphs,
in preparation.

\bibitem{RobSeyGM9}N.~Robertson and P.~D.~Seymour,
Graph Minors IX. Disjoint crossed paths,
\JCTB\ {\bf 49} (1990), 40--77.

\bibitem{RobSeyThoCubic} N.~Robertson, P.~D.~Seymour and R.~Thomas,
Excluded minors in cubic graphs, manuscript.

\bibitem{SeyDisj} P. D. Seymour, Disjoint paths in graphs,
{\it Discrete Math.} {\bf 29} (1980), 293-309.

\bibitem{Shi} Y. Shiloach,
A polynomial solution to the undirected two paths problem,
{\it J.~Assoc.\ Comp.\ Machinery}, {\bf27}, (1980), 445-456.

\bibitem{ThoSurvey}R.~Thomas.  Recent excluded minor theorems for graphs. {\it Surveys in combinatorics,  London Math. Soc. Lecture Note Ser.} {\bf 267} (1999),  201--222.

\bibitem{ThoThoTutte} R.~Thomas and J.~Thomson,
Excluding minors in nonplanar graphs of girth five,
{\it\CPC} {\bf9} (2000), 573--585.

\bibitem{Tho2link} C. Thomassen, 2-linked graphs,
{\it Europ.\ J.\ Combinatorics}  {\bf1} (1980), 371--378.

\bibitem{TutHowto}W.~T.~Tutte,
How to draw a graph,
{\sl Proc.\ London Math.\ Soc.\ \bf 13} (1963), 743--768.

\bibitem{Tut66}W.~T.~Tutte, On the algebraic theory of graph colorings,
\JCTB\ {\bf 1} (1966), 15--50.
%3-edge-coloring and 4-flow conjecture, $3$-flow conjecture

\bibitem{WhiCongr} H.~Whitney,
Congruent graphs and the connectivity of graphs,
{\sl Amer.~J.\ Math.\ \bf 54} (1932), 150--168.


